Question Answering as Programming for Solving Time-Sensitive Questions

Question answering plays a pivotal role in human daily life because it involves our acquisition of knowledge about the world. However, due to the dynamic and ever-changing nature of real-world facts, the answer can be completely different when the time constraint in the question changes. Recently, Large Language Models (LLMs) have shown remarkable intelligence in question answering, while our experiments reveal that the aforementioned problems still pose a significant challenge to existing LLMs. This can be attributed to the LLMs' inability to perform rigorous reasoning based on surface-level text semantics. To overcome this limitation, rather than requiring LLMs to directly answer the question, we propose a novel approach where we reframe the $\textbf{Q}$uestion $\textbf{A}$nswering task $\textbf{a}$s $\textbf{P}$rogramming ($\textbf{QAaP}$). Concretely, by leveraging modern LLMs' superior capability in understanding both natural language and programming language, we endeavor to harness LLMs to represent diversely expressed text as well-structured code and select the best matching answer from multiple candidates through programming. We evaluate our QAaP framework on several time-sensitive question answering datasets and achieve decent improvement, up to $14.5$% over strong baselines. Our codes and data are available at https://github.com/TianHongZXY/qaap

==> tables/abla_diff_lm_for_check_match.tex <==
\begin{table}[tp]
\centering
\begin{adjustbox}{max width=0.49\textwidth}
\small
\begin{tabular}{lc|ccc}
\toprule
% \noalign{\hrule height 1.2pt}
\multirow{2}{*}{Method}    & \multirow{2}{*}{$K_{e}$} & \multicolumn{2}{c}{TimeQA} & \multirow{2}{*}{TimeQuestions} \\ 
 &  &  Easy  & Hard & \\
 %  golden K_{e} 要不要重新划分成一行新栏
\midrule
CoT   &   \xmark    &   24.6   & 21.7  &   28.2  \\
CoT-variant &  \cmark    & 22.0  & 18.5  &   30.6 \\ 
% \rowcolor{aliceblue!60} 
Ours  & \cmark  & \textbf{41.0}    & \textbf{34.1}  &  \textbf{31.5}  \\
\midrule
CoT-variant$^*$ & \cmark & 48.0 & 33.7  &   - \\
Ours$^*$  & \cmark  & \textbf{53.0} & \textbf{47.2}  &  -  \\
\bottomrule
% \noalign{\hrule height 1.2pt}
\end{tabular}
\end{adjustbox}
\caption{EM scores on three datasets. $K_{e}$ refers to external knowledge. $^*$ indicates given golden paragraphs containing ground truth.}
\label{table:abla_diff_lm_for_check_match}
\end{table}

==> tables/case_study.tex <==
\definecolor{darkGreen}{rgb}{0.2,0.5,0.2}
\begingroup
\begin{table*}[h]
    \centering
    \small
    % \begin{tabular}{p{\linewidth}}
    \begin{tabular}{p{0.93\linewidth}}
        \toprule
        \vspace{-2mm}
        \textbf{\textsc{Question:}} Who was Arnulf Øverland 's spouse \textbf{\color{temporalcolor}{between May 1944 and Jun 1944}}? \\
        \vspace{-1mm}
        \textbf{\textsc{Context}:} Arnulf Øverland was a Norwegian author, poet, and critic. \\
        %
        ... \\
        %
        Personal life . \textbf{\color{blue}{In 1918}} he had married the singer \textbf{\color{red}{Hildur Arntzen}} ( 1888–1957 ) . Their marriage was dissolved \textbf{\color{blue}{in 1939}} . \textbf{\color{temporalcolor}{In 1940}} , he married \textbf{\color{darkGreen}{Bartholine Eufemia Leganger}} ( 1903–1995 ) . They separated shortly after , and were officially divorced \textbf{\color{temporalcolor}{in 1945}}.
        Øverland was married to journalist \textbf{\color{red}{Margrete Aamot Øverland}} ( 1913–1978 ) \textbf{\color{blue}{during June 1945}}. \\
        \vspace{-1mm}
        \textbf{\textsc{Golden Answer:}} \textbf{\color{darkGreen}{Bartholine Eufemia Leganger}} \\
        % In 1946 , the Norwegian Parliament arranged for Arnulf and Margrete Aamot Øverland to reside at the Grotten . He lived there until his death in 1968 and she lived there for another ten years until her death in 1978 . Arnulf Øverland was buried at Vår Frelsers Gravlund in Oslo . Joseph Grimeland designed the bust of Arnulf Øverland ( bronze , 1970 ) at his grave site .
        \midrule
        \vspace{-2mm}
        \textbf{\textsc{CoT (without context):}} Arnulf Øverland was a Norwegian author, poet, and social commentator. He was married to pianist and composer \textbf{\color{red}{Harriet Cohen}} from 1937 until her death in 1967. There is no answer. \xmark{} \\
        %
        \midrule
        \vspace{-2mm}
        \textbf{\textsc{CoT-variant$^*$:}} <CONTEXT>\\
        Is the answer in the context? Yes \\ Answer: \textbf{\color{red}{Margrete Aamot Øverland}} \xmark{} \\
        \midrule
        \vspace{-2mm}
        \textbf{\textsc{ReAct:}} Thought 1: I need to search Arnulf Øverland and find out who his spouse was between May 1944 and Jun 1944.\\ Action 1: Search[Arnulf Øverland]\\ Observation 1: Arnulf Øverland was a Norwegian author, poet, and critic. He was married to the author and translator Berit Ås from 1945 until his death in 1968. 
        During the German occupation of Norway from 1940 in World War II , he wrote to inspire the Norwegian resistance movement .\\ Thought 2: The paragraph does not tell who Arnulf Øverland's spouse was between May 1944 and Jun 1944, maybe I can look up the years between 1944 and 1944. First I can look up ``1944''.\\ Action 2: Lookup[1944]\\ Observation 2: No more results.\\  Thought 3: There is no results for ``1944'', let's look up ``spouse''.\\ Action 3: Lookup[spouse]\\ Observation 3: No more results.\\ Thought 4: The passage does not tell who Arnulf Øverland's spouse was between May 1944 and Jun 1944.\\ Action 4: Finish[] \xmark{} \\
        \midrule
        \vspace{-2mm}
        \textbf{\textsc{QAaP:}} Question Parsing: 
        \begin{verbatim}
```python
query = {"subject": "Arnulf Øverland", "relation": "spouse", "object": None, "time": {"start": da
tetime(1944, 5, 1), "end": datetime(1944, 6, 30)}}
answer_key = "object"
```
\end{verbatim}
% 
<CONTEXT>\\
Extract information relevant to the query:
\begin{verbatim}
```python
information.append({"subject": "Arnulf Øverland", "relation": "spouse", "object": "Hildur Arntz
en", "time": {"start": datetime(1918, 1, 1), "end": datetime(1939, 12, 31)}})

information.append({"subject": "Arnulf Øverland", "relation": "spouse", "object": "Bartholine Eu
femia Leganger", "time":{"start": datetime(1940, 1, 1), "end": datetime(1945, 12, 31)}})

information.append({"subject": "Arnulf Øverland", "relation": "spouse", "object": "Margrete Aamo
t Øverland", "time": {"start": datetime(1945, 6, 1), "end": None}})
``` 
\end{verbatim}\\
\bottomrule
    \end{tabular}
    \caption{
    Examples of correct and incorrect answers obtained with different methods on TimeQA.
    }
    \label{table:case_study}
\end{table*}
\endgroup


